Infinite-Fidelity Coregionalization for Physical Simulation

Multi-fidelity modeling and learning are important in physical simulation-related applications. It can leverage both low-fidelity and high-fidelity examples for training so as to reduce the cost of data generation while still achieving good performance. While existing approaches only model finite, discrete fidelities, in practice, the fidelity choice is often continuous and infinite, which can correspond to a continuous mesh spacing or finite element length. In this paper, we propose Infinite Fidelity Coregionalization (IFC). Given the data, our method can extract and exploit rich information within continuous, infinite fidelities to bolster the prediction accuracy. Our model can interpolate and/or extrapolate the predictions to novel fidelities, which can be even higher than the fidelities of training data. Specifically, we introduce a low-dimensional latent output as a continuous function of the fidelity and input, and multiple it with a basis matrix to predict high-dimensional solution outputs. We model the latent output as a neural Ordinary Differential Equation (ODE) to capture the complex relationships within and integrate information throughout the continuous fidelities. We then use Gaussian processes or another ODE to estimate the fidelity-varying bases. For efficient inference, we reorganize the bases as a tensor, and use a tensor-Gaussian variational posterior to develop a scalable inference algorithm for massive outputs. We show the advantage of our method in several benchmark tasks in computational physics.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


\cmt{
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
	justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
	\item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
	\item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
	\item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
}


\begin{enumerate}
	
	
	\item For all authors...
	\begin{enumerate}
		\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
		\answerYes{}
		\item Did you describe the limitations of your work?
		\answerYes{}
		\item Did you discuss any potential negative societal impacts of your work?
		\answerNA{}
		\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
		\answerYes{}
	\end{enumerate}
	
	
	\item If you are including theoretical results...
	\begin{enumerate}
		\item Did you state the full set of assumptions of all theoretical results?
		\answerNA{}
		\item Did you include complete proofs of all theoretical results?
		\answerNA{}
	\end{enumerate}
	
	
	\item If you ran experiments...
	\begin{enumerate}
		\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
		\answerYes{}
		\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
		\answerYes{}
		\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
		\answerYes{}
		\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
		\answerYes{}
	\end{enumerate}
	
	
	\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
	\begin{enumerate}
		\item If your work uses existing assets, did you cite the creators?
		\answerYes{}
		\item Did you mention the license of the assets?
		\answerNA{}
		\item Did you include any new assets either in the supplemental material or as a URL?
		\answerNA{}
		\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
		\answerNA{}
		\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
		\answerNA{}
	\end{enumerate}
	
	
	\item If you used crowdsourcing or conducted research with human subjects...
	\begin{enumerate}
		\item Did you include the full text of instructions given to participants and screenshots, if applicable?
		\answerNA{}
		\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
		\answerNA{}
		\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
		\answerNA{}
	\end{enumerate}
	
	
\end{enumerate}

==> exp.tex <==
%\vspace{-0.05in}
\section{Experiment}
%\vspace{-0.1in}
%Burgers [16, 24,32,64]; TopOpt [50,60,70,80]; NS [32,48,64,80] * (20 time steps)
\subsection{Predicting Solution Fields of Partial Differential Equations}
%\vspace{-0.1in}
We first tested \ours for predicting the solution fields of several benchmark PDEs in computational physics, including Poisson's, Heat and Burger's equations~\citep{olsen2011numerical}.  To collect the training data, we run the numerical solvers with several meshes. Denser meshes generate examples of higher fidelities. The output vector comprises of the solution values on the whole mesh. For instance, a mesh of size $50 \times 50$ corresponds to an output vector of $2,500$ dimensions.  For Poisson's and Heat equation, we generated training examples of four fidelities, using $8 \times 8$, $16 \times 16$, $32 \times 32$ and $64 \times 64$ meshes, respectively. For Burger's equation, we used $16 \times 16$, $24 \times 24$, $32 \times 32$ and $64 \times 64$ meshes to generate four-fidelity training data. For all PDEs, the number of training examples for each fidelity (from the lowest to highest) is $100$, $50$, $20$, and $5$, respectively. For testing, we generated 128 examples with the highest fidelity. Both the training and test inputs were uniformly sampled from the domain (but they do not overlap). The input includes boundary and/or PDE parameters. The input dimension for Poisson's, Heat and Burger's equation is five, three and one, respectively. Hence, the task is to learn  low-to-high mappings from data. The data generation details are given in Appendix. 

\noindent\textbf{Competing Methods.} We compared with the following state-of-the-art multi-fidelity high-dimensional output learning methods. (1) DRC~\citep{xing2021deep}, deep residual coregionalization, which performs LMC on the residual error of the predictions from the lower fidelities. The final prediction is the summation of the LMC prediction across all the fidelities. See Sec. XXX. (2) MFHoGP~\citep{wang2021multi}, which uses a matrix GP prior to construct a nonlinear coregionalization (NC)  model, and connects multiple NC models for multi-fidelity learning, one for each fidelity. To capture the correlation between successive fidelities, the matrix GP prior in each fidelity incorporates the latent output in the previous fidelity as a part of the input. (3) DMF~\citep{li2020deep}, a multi-fidelity learning model based on a stack of deep neural networks (NNs), where each NN is for one fidelity. To synergize different fidelities,  the latent output of each NN is fed into the NN for the next fidelity. The high-dimensional prediction in each fidelity is made by a linear projection of the latent output.  In addition, to verify \ours can indeed better integrate information of different fidelities, we also tested (4) SF, the single-fidelity degeneration of our model, where the prediction is $\f(\x)= \B_0 \h_0(\x)$, where $\B_0$ is a static basis matrix, and $\h_0(\cdot )$ is a neural network. SF uses all the training examples without differentiation.  We denote our ODE based method using GP prior over the basis matrix by (5) \ours-GPODE and latent ODE over each basis element by (6) \ours-ODE$^2$. 

\noindent\textbf{Settings and Results.} All the methods were implemented by PyTorch~\citep{raissi2019physics}, except that DRC was implemented by MATLAB. For GP related models, including DRC, MFHoGP and \ours-GPODE, we used the square exponential (SE) kernel. The length-scale parameter was initialized to one. For our method, each NN component ($\bphi$, $\bbeta$, and $\gamma$ in Eq. XX, XX and XX) employed two hidden layers with \texttt{tanh} as the activation function. To handle continuous (infinite) fidelities, we mapped the lowest fidelity to $m=0$, and highest to $m=1$. For convenience, we use a linear mapping from the mesh size to the fidelity value $m$. Note that, the (possible) nonlinear relationship across the fidelities can still be captured by our neural ODE component over $m$ (see XXX).    For DMF, we also used two hidden layers for each NN, and \textit{tanh} as the activation, which is consistent with the setting in~\citep{li2020deep}. The number of neurons per layer was chosen from $\{10, 20, 30, 40, 50, 60\}$. We found that more layers for both our method and DMF did not improve the predictive performance. In addition, other choices of the activation function, such as ReLU and LeakyReLu worsened the performance. This is consistent with the typical activation function choice in physics-informed neural networks~\citep{raissi2019physics}. We ran ADAM~\citep{kingma2014adam} to train all the models, except DRC, which uses L-BFGS to training the latent functions (the maximum number of iterations was set to 1K). We used ReduceLROnPlateau scheduler to adjust the learning rate from $[10^{-3}, 10^{-2}]$. We set the maximum number of epochs to 5000, which ensures the convergence of every method. We verified the dimension of the latent output from \{5, 10, 15, 20\}. For each setting, we repeated the experiment for five times (training/test data generation and learning). The average root-mean-square-error (RMSE) and the standard deviation of each method are reported in Fig. XX

As we can see, both   \ours-GPODE and \ours-ODE$^2$ consistently outperform all the competing methods by a large margin. The prediction errors of \ours-GPODE and \ours-ODE$^2$ are close,  showing that they achieve similar predictive performance. The both versions of \ours greatly outperforms SF --- the single-fidelity degeneration, and in most case SF is also worse than the competing finite fidelity models. This together demonstrates the advantage of our infinite-fidelity modeling, and the improvement is indeed from more effective usage of the training information across different fidelities. 

\cmt{
\begin{figure*}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{ccc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/new/Burgers_legend.pdf}
			\caption{\small \textit{Burgers}}
		\end{subfigure} &
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/new/Heat2.pdf}
			\caption{\small \textit{Heat}}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/new/Poisson2.pdf}
			\caption{\small \textit{Poisson}}
		\end{subfigure}\\
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/new/Poisson3.pdf}
			\caption{\small \textit{Poisson-3}}\label{fig:solving-po-3fid}
		\end{subfigure} &
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			%\includegraphics[width=\textwidth]{./figs/rmse_Lbracket-trunc.pdf}
			\includegraphics[width=\textwidth]{./figs/new/Lbracket.pdf}
			\caption{\small \textit{Topology structure optimization}} \label{fig:tpo}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			%\includegraphics[width=\textwidth]{./figs/rmse_Navier-trunc.pdf}
			\includegraphics[width=\textwidth]{./figs/new/Navier.pdf}
			\caption{\small \textit{Fluid dynamics}}\label{fig:ns}
		\end{subfigure}
	\end{tabular}
	%\vspace{-0.1in}
	\caption{\small Normalized root-mean-square error (nRMSE) \textit{vs.} total cost (running time) in active learning. The results are averaged from five runs. The shaded regions indicate the standard deviations.} \label{fig:al-acc}
	\vspace{-0.2in}
\end{figure*}
}

\cmt{
\setlength{\columnsep}{5pt}
\begin{figure}[!htb]
	\centering
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_ground_v1.eps}
		\caption{\small Ground Truth}
		\label{fig:tpo-gt}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_mutual_v1.eps}
		\caption{\small \ours}
		\label{fig:tpo-ours}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_dropout_v1.eps}
		\caption{\small Dropout-latent}
		\label{fig:tpo-dropout}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_bald_v1.eps}
		\caption{\small MF-BALD}
		\label{fig:tpo-bald}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/new/pdv.eps}
		\caption{\small MF-PredVar}
		\label{fig:tpo-pdv}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_full_random_v1.eps}
		\caption{\small MF-Random}
		\label{fig:tpo-random}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_fix_random_f1_v1.eps}
		\caption{\small Random-F1}
		\label{fig:tpo-random-1}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_fix_random_f2_v1.eps}
		\caption{\small Random-F2}
		\label{fig:tpo-random-2}
	\end{subfigure}
	%\vspace{-0.1in}
	\caption{\small The predicted topology structures for $8$ loads. All the active learning approaches started with the same training set (10 fidelity-1 and 2 fidelity-2 examples), and ran with $100$ queries.}
	\label{fig:pred-top-structure}
	%\vspace{-0.2in}
\end{figure}
}
\cmt{
The inferior performance of {MF-BALD} and {MF-PredVar} to \ours indicates that the straightforward extension of BALD and predictive variance can be suboptimal, which  might partly because they miss the influence of the low-fidelity training examples on the final predictions (\ie at the highest fidelity). How to better generalize BALD and PredVar to the multi-fidelity setting remains an open problem. % In addition, \texttt{MF-PredVar} ignores the output correlations, which lead to worse calibrated uncertainty of the outputs and affect 
%The worse performance of \texttt{Dropout-latent} than \ours implies that our structural variational inference can give a better posterior estimation for the latent outputs than the stochastic estimations constructed from the dropout samples. 
Overall,  these results have demonstrated the advantage of our deep multi-fidelity active learning  approach. 
%\vspace{-0.1in}
}
\subsection{Topology Optimization}
%\vspace{-0.1in}

Next, we applied \ours in predicting the optimal topology design structures. Topology optimization (TO) is an important task in engineering design and manufacturing.  In general,  given the input constraint, \eg external force, our goal is to find a layout of the give materials (\eg alloys) that maximizes/minimizes the property of interest, \eg stiffness. The standard TO solves a constraint optimization problem that includes a compliance objective and total volume constraint~\citep{sigmund1997design}. The computation of objective often demand for solving associated PDEs, and hence is quite computationally expensive. Hence, we want to train a surrogate model to predict the optimal structure directly, given the input constraints. We considered the design problem in~\citep{keshavarzzadeh2018parametric}, where we aim to find a structure in an L-shape domain (discretized in $[0,1 ] \times [0, 1]$), which can achieve the maximum stiffness under a load on the bottom right half. The load (input) is expressed by the location (in $[0.5, 1]$) and angle (in $[0, \frac{\pi}{2}]$). The strength of the load is fixed. To find the optimal structure, we need to run a numerical solver.  To train the surrogate model, we generated training examples with four fidelities, corresponding to $50 \times 50$, $60 \times 60$, $70 \times 70$ and $80 \times 80$ meshes. Again, we generated $100$, $50$, $20$, $5$ for each fidelity, and $128$ examples at the highest fidelity for testing. We repeated the experiment for five times. The average RMSE and standard deviation are shown in Fig. XX. As we can see, \ours-GPODE and \ours-ODE$^2$ achieve much higher prediction accuracy than all the competing methods in all the cases. It is interesting to see that the performance of our method kept improving with the increase of the latent output dimension. This is might because more latent outputs can summarize and propagate the fidelity information more comprehensively and accurately. 

%\vspace{-0.15in}
\subsection{Computational Fluid Dynamics}
%\vspace{-0.1in}
Third, we applied \ours in predicting the simulation results of computational fluid dynamics. Specifically, we considered a flow driven by rectangular boundaries~\citep{bozeman1973numerical}. The rectangular is in the domain $[0, 1] \times [0, 1]$. Each of the four boundaries has a prescribed velocity. We were interested in predicting the pressure field of the flow along with time in $[0, 10]$. The spatial-temporal field can be computed by solving the incompressive Navier-Stokes (NS) equations~\citep{chorin1968numerical}, which is known to be costly due to the complex behaviors under large Renolds numbers. We simulated training examples of four fidelities, with spatial meshes of size $32 \times 32$, $48 \times 48$, $64 \times 64$ and $80 \times 80$ respectively. The number of time steps was set to $20$. Hence, the output dimension (at the highest fidelity) is 128K.  Similar to the previous experiments, we collected 100, 50, 20, and 5 examples for each fidelity, and 128 examples at the highest fidelity for testing. We ran every method and examined the prediction accuracy. We repeated the experiment for five times and report the average RMSE in Fig. XX. We can see that, consistent with the previous comparison results,  \ours (both versions) greatly outperforms all the competing multi-fidelity and single-fidelity methods, confirming the advantage of \ours in predicting complex physical simulation results.  

\subsection{Interpolation and Extrapolation in Fidelities}

Since our method predicts the output as a function of the (continuous) fidelity,  it can predict solution fields at arbitrary fidelities that are different from the training fidelities, namely, interpolation and extrapolation. Note that, the current finite fidelity approaches lack a mechanism to make such predictions. To examine the performance of our model in interpolating and extrapolating the fidelity of  solution prediction, we tested on Poisson's and Heat equation. We generated the four-fidelity training data, including $256$, $128$, $64$, and $32$ examples for the first, second, third and fourth fidelity. The corresponding mesh size is $8 \times 8$, $16 \times 16$, $32 \times 32$ and $64 \times 64$, respectively. The lowest fidelity is $m=0$, and highest $m=1$. We then trained our model, and predicted the solution at $m>1$, which corresponds to denser meshes. For example, $m=1.29, 1.57, 2.14$ correspond to the mesh size $80 \times 80$, $96 \times 96$ and $128 \times 128$.  We viewed the ideal solution as solved using the $128 \times 128$ mesh, with which we generated 256 test examples. We then varied $m \in [0, 2.14]$, and examined the prediction error of \ours at various fidelities. The results are shown in Fig. XX. As we can see, within the range of the training fidelity ($m \le 1$), the prediction error of  \ours-GPODE is consistently smaller than that of  \ours-ODE$^2$, especially at very low fidelities. The best prediction error of \ours-GPODE is achieved at $m=1$, \ie the highest training fidelity. When $m>1$, the performance of \ours-GPODE drops evidently. By contrast, while when $m<1$, the prediction error of \ours-ODE$^2$ is slightly worse than \ours-GPODE, when $m>1$, the performance of \ours-ODE$^2$ keeps improving. At the end $m=2.14$, the prediction error is even better than the best error of \ours-GPODE. It shows that \ours-GPODE is better in interpolation but \ours-ODE$^2$ is promising in extrapolation. This might be attributed to the GP prior used \ours-GPODE, which is known to interpolate well yet not good at extrapolation. The improved extrapolation performance of \ours-ODE$^2$ can be particularly useful in practice. It allows us to train the surrogate model only using relatively low-fidelity examples, but we can still expect to extrapolate predictions to higher fidelities. Therefore, we can avoid generating those higher-fidelity examples for training and hence greatly reduce the cost. 



==> exp_shibo.tex <==
%\vspace{-0.05in}
\section{Experiment}
%\vspace{-0.1in}
%Burgers [16, 24,32,64]; TopOpt [50,60,70,80]; NS [32,48,64,80] * (20 time steps)
\subsection{Predicting Solution Fields of Partial Differential Equations}
%\vspace{-0.1in}
We first tested \ours for predicting the solution fields of several benchmark PDEs in computational physics, including Poisson's, Heat and Burger's equations~\citep{olsen2011numerical}.  To collect the training data, we run the numerical solvers with several meshes. Denser meshes give examples of higher fidelities. The output vector comprises of the solution values on the whole mesh. For instance, a mesh of size $50 \times 50$ corresponds to an output vector of $2,500$ dimensions.  For Poisson's and Heat equations, we generated training examples of four fidelities, using $8 \times 8$, $16 \times 16$, $32 \times 32$ and $64 \times 64$ meshes, respectively. For Burger's equation, we used $16 \times 16$, $24 \times 24$, $32 \times 32$ and $64 \times 64$ meshes to generate four-fidelity training data. For all PDEs, the number of training examples for each fidelity (from the lowest to highest) is $100$, $50$, $20$, and $5$, respectively. For testing, we generated 128 examples with the highest fidelity. Both the training and test inputs were uniformly sampled from the domain (but they do not overlap). The input includes boundary and/or PDE parameters. The input dimension for Poisson's, Heat and Burger's equation is five, three and one, respectively. Hence, the task is to learn an low-to-high mapping from data. The data generation details are supplemented in Appendix. 

\noindent\textbf{Competing Methods.} We compared with the following state-of-the-art multi-fidelity high-dimensional output learning methods. (1) DRC~\citep{xing2021deep}, deep residual coregionalization, which performs LMC on the residual error of the predictions from the lower fidelities. The final prediction is the summation of the LMC prediction across all the fidelities. See Sec. XXX. (2) MFHoGP~\citep{wang2021multi}, which uses a matrix GP prior to construct a nonlinear coregionalization (NC)  model, and connects multiple NC models for multi-fidelity learning, one for each fidelity. To capture the correlation between successive fidelities, the matrix GP prior in each fidelity incorporates the latent output in the previous fidelity as a part of the input. (3) DMF~\citep{li2020deep}, a multi-fidelity learning model based on a stack of deep neural networks (NNs), where each NN is for one fidelity. To synergize different fidelities,  the latent output of each NN is fed into the NN for the next fidelity. The high-dimensional prediction in each fidelity is made by a linear projection of the latent output.  In addition, to verify \ours can indeed better integrate information of different fidelities, we also tested (4) SF, the single-fidelity degeneration of our model, where the prediction is $\f(\x)= \B_0 \h_0(\x)$, where $\B_0$ is a static basis matrix, and $\h_0(\cdot )$ is a neural network. SF uses all the training examples without differentiation.  We denote our ODE based method using GP prior over the basis matrix by (5) \ours-GPODE and latent ODE over each basis element by (6) \ours-ODE$^2$. 

\noindent\textbf{Settings and Results.} All the methods were implemented by PyTorch~\citep{raissi2019physics}, except that DRC was implemented by MATLAB. For GP related models, including DRC, MFHoGP and \ours-GPODE, we used the square exponential (SE) kernel. The length-scale parameter was initialized to one. For our method, each NN component ($\bphi$, $\bbeta$, and $\gamma$ in Eq. XX, XX and XX) employed two hidden layers with \texttt{tanh} as the activation function. To handle continuous (infinite) fidelities, we mapped the lowest fidelity to $m=0$, and highest to $m=1$. For convenience, we use a linear mapping from the mesh size to the fidelity value $m$. Note that, the (possible) nonlinear relationship across the fidelities can still be captured by our neural ODE component over $m$ (see XXX).    For DMF, we also used two hidden layers for each NN, and \textit{tanh} as the activation, which is consistent with the setting in~\citep{li2020deep}. The number of neurons per layer was chosen from $\{10, 20, 30, 40, 50, 60\}$. We found that more layers for both our method and DMF did not improve the predictive performance. In addition, other choices of the activation function, such as ReLU and LeakyReLu worsened the performance. This is consistent with the typical activation function choice in physics-informed neural networks~\citep{raissi2019physics}. We ran ADAM~\citep{kingma2014adam} to train all the models, except DRC, which uses L-BFGS to training the latent functions (the maximum number of iterations was set to 1K). We used ReduceLROnPlateau scheduler to adjust the learning rate from $[10^{-3}, 10^{-2}]$. We set the maximum number of epochs to 5000, which ensures the convergence of every method. We verified the dimension of the latent output from \{5, 10, 15, 20\}. For each setting, we repeated the experiment for five times (training/test data generation and learning). The average root-mean-square-error (RMSE) and the standard deviation of each method are reported in Fig. XX

As we can see, both   \ours-GPODE and \ours-ODE$^2$ consistently outperform all the competing methods by a large margin. The prediction errors of \ours-GPODE and \ours-ODE$^2$ are close,  showing that they achieve similar predictive performance. The both versions of \ours greatly outperforms SF --- the single-fidelity degeneration, and in most case SF is also worse than the competing finite fidelity models. This together demonstrates the advantage of our infinite-fidelity modeling, and the improvement is indeed from more effective usage of the training information across different fidelities. 

\begin{figure*}
	\centering
	\setlength\tabcolsep{0pt}
	\includegraphics[width=0.7\textwidth]{./figs2/legend.pdf}
	\begin{tabular}[c]{ccccc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.2\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs2/rmse_Poisson.pdf}
			\caption{\small \textit{Poisson}}
		\end{subfigure}
	   &
		\begin{subfigure}[t]{0.205\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs2/rmse_Heat.pdf}
			\caption{\small \textit{Heat}}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.2\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs2/rmse_Burgers.pdf}
			\caption{\small \textit{Burgers}}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.2\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs2/rmse_TopOpt.pdf}
			\caption{\small \textit{TopOpt}}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.2\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs2/rmse_NavierStockPRec.pdf}
			\caption{\small \textit{NS}}
		\end{subfigure}
	\end{tabular}
	%\vspace{-0.1in}
	\caption{nRMSE} \label{fig:nrmse}
	\vspace{-0.2in}
\end{figure*}

\begin{figure*}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{cc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.48\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs2/errors_Poisson.pdf}
			\caption{\small \textit{Poisson}}
		\end{subfigure} 
		&
		\begin{subfigure}[t]{0.48\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs2/errors_NavierStockPRec.pdf}
			\caption{\small \textit{NS $t=10.0$}}
		\end{subfigure}
	\end{tabular}
	%\vspace{-0.1in}
	\caption{\small Examples of the prediction error field. For NS, we only display the pressure field when t=10.0(the last episode). All the error fields of compared methods are normalized to the same scale $[0.0, \max(y_i)]$} \label{fig:error_field}
	\vspace{-0.2in}
\end{figure*}

\begin{figure*}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{cc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.48\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs2/extrap_err_Poisson.pdf}
			\caption{\small \textit{Poisson}}
		\end{subfigure} 
		&
		\begin{subfigure}[t]{0.48\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs2/extrap_err_Heat.pdf}
			\caption{\small \textit{Heat}}
		\end{subfigure}
	\end{tabular}
	%\vspace{-0.1in}
	\caption{\small Interpolation/Extrapolation errors for Poisson and Heat with number of bases 20} \label{fig:extrap_errbar}
	\vspace{-0.2in}
\end{figure*}

\begin{figure*}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{cc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.48\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs2/extrap_Poisson.pdf}
			\caption{\small \textit{Poisson}}
		\end{subfigure} 
		&
		\begin{subfigure}[t]{0.48\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs2/extrap_Heat.pdf}
			\caption{\small \textit{Heat}}
		\end{subfigure}
	\end{tabular}
	%\vspace{-0.1in}
	\caption{\small Examples of interpolation/extrapolation of Poisson and Heat. fidelity 8,32,64,96,128} \label{fig:extrap_examples}
	\vspace{-0.2in}
\end{figure*}

\cmt{
\begin{figure*}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{ccc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/new/Burgers_legend.pdf}
			\caption{\small \textit{Burgers}}
		\end{subfigure} &
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/new/Heat2.pdf}
			\caption{\small \textit{Heat}}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/new/Poisson2.pdf}
			\caption{\small \textit{Poisson}}
		\end{subfigure}\\
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/new/Poisson3.pdf}
			\caption{\small \textit{Poisson-3}}\label{fig:solving-po-3fid}
		\end{subfigure} &
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			%\includegraphics[width=\textwidth]{./figs/rmse_Lbracket-trunc.pdf}
			\includegraphics[width=\textwidth]{./figs/new/Lbracket.pdf}
			\caption{\small \textit{Topology structure optimization}} \label{fig:tpo}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			%\includegraphics[width=\textwidth]{./figs/rmse_Navier-trunc.pdf}
			\includegraphics[width=\textwidth]{./figs/new/Navier.pdf}
			\caption{\small \textit{Fluid dynamics}}\label{fig:ns}
		\end{subfigure}
	\end{tabular}
	%\vspace{-0.1in}
	\caption{\small Normalized root-mean-square error (nRMSE) \textit{vs.} total cost (running time) in active learning. The results are averaged from five runs. The shaded regions indicate the standard deviations.} \label{fig:al-acc}
	\vspace{-0.2in}
\end{figure*}
}

\cmt{
\setlength{\columnsep}{5pt}
\begin{figure}[!htb]
	\centering
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_ground_v1.eps}
		\caption{\small Ground Truth}
		\label{fig:tpo-gt}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_mutual_v1.eps}
		\caption{\small \ours}
		\label{fig:tpo-ours}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_dropout_v1.eps}
		\caption{\small Dropout-latent}
		\label{fig:tpo-dropout}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_bald_v1.eps}
		\caption{\small MF-BALD}
		\label{fig:tpo-bald}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/new/pdv.eps}
		\caption{\small MF-PredVar}
		\label{fig:tpo-pdv}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_full_random_v1.eps}
		\caption{\small MF-Random}
		\label{fig:tpo-random}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_fix_random_f1_v1.eps}
		\caption{\small Random-F1}
		\label{fig:tpo-random-1}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_fix_random_f2_v1.eps}
		\caption{\small Random-F2}
		\label{fig:tpo-random-2}
	\end{subfigure}
	%\vspace{-0.1in}
	\caption{\small The predicted topology structures for $8$ loads. All the active learning approaches started with the same training set (10 fidelity-1 and 2 fidelity-2 examples), and ran with $100$ queries.}
	\label{fig:pred-top-structure}
	%\vspace{-0.2in}
\end{figure}
}
\cmt{
The inferior performance of {MF-BALD} and {MF-PredVar} to \ours indicates that the straightforward extension of BALD and predictive variance can be suboptimal, which  might partly because they miss the influence of the low-fidelity training examples on the final predictions (\ie at the highest fidelity). How to better generalize BALD and PredVar to the multi-fidelity setting remains an open problem. % In addition, \texttt{MF-PredVar} ignores the output correlations, which lead to worse calibrated uncertainty of the outputs and affect 
%The worse performance of \texttt{Dropout-latent} than \ours implies that our structural variational inference can give a better posterior estimation for the latent outputs than the stochastic estimations constructed from the dropout samples. 
Overall,  these results have demonstrated the advantage of our deep multi-fidelity active learning  approach. 
%\vspace{-0.1in}
}
\subsection{Topology Optimization}
%\vspace{-0.1in}

Next, we applied \ours in predicting the optimal topology design structures. Topology optimization (TO) is an important task in engineering design and manufacturing.  In general,  given the input constraint, \eg external force, our goal is to find a layout of the give materials (\eg alloys) that maximizes/minimizes the property of interest, \eg stiffness. The standard TO solves a constraint optimization problem that includes a compliance objective and total volume constraint~\citep{sigmund1997design}. The computation of objective often demand for solving associated PDEs, and hence is quite computationally expensive. Hence, we want to train a surrogate model to predict the optimal structure directly, given the input constraints. We considered the design problem in~\citep{keshavarzzadeh2018parametric}, where we aim to find a structure in an L-shape domain (discretized in $[0,1 ] \times [0, 1]$), which can achieve the maximum stiffness under a load on the bottom right half. The load (input) is expressed by the location (in $[0.5, 1]$) and angle (in $[0, \frac{\pi}{2}]$). The strength of the load is fixed. To find the optimal structure, we need to run a numerical solver.  To train the surrogate model, we generated training examples with four fidelities, corresponding to $50 \times 50$, $60 \times 60$, $70 \times 70$ and $80 \times 80$ meshes. Again, we generated $100$, $50$, $20$, $5$ for each fidelity, and $128$ examples at the highest fidelity for testing. We repeated the experiment for five times. The average RMSE and standard deviation are shown in Fig. XX. As we can see, \ours-GPODE and \ours-ODE$^2$ achieve much higher prediction accuracy than all the competing methods in all the cases. It is interesting to see that the performance of our method kept improving with the increase of the latent output dimension. This is might because more latent outputs can summarize and propagate the fidelity information more comprehensively and accurately. 

%\vspace{-0.15in}
\subsection{Computational Fluid Dynamics}
%\vspace{-0.1in}
Third, we applied \ours in predicting the simulation results of computational fluid dynamics. Specifically, we considered a flow driven by rectangular boundaries~\citep{bozeman1973numerical}. The rectangular is in the domain $[0, 1] \times [0, 1]$. Each of the four boundaries has a prescribed velocity. We were interested in predicting the pressure field of the flow along with time in $[0, 10]$. The spatial-temporal field can be computed by solving the incompressive Navier-Stokes (NS) equations~\citep{chorin1968numerical}, which is known to be costly due to the complex behaviors under large Renolds numbers. We simulated training examples of four fidelities, with spatial meshes of size $32 \times 32$, $48 \times 48$, $64 \times 64$ and $80 \times 80$ respectively. The number of time steps was set to $20$. Hence, the output dimension (at the highest fidelity) is 128K.  Similar to the previous experiments, we collected 100, 50, 20, and 5 examples for each fidelity, and 128 examples at the highest fidelity for testing. We ran every method and examined the prediction accuracy. We repeated the experiment for five times and report the average RMSE in Fig. XX. We can see that, consistent with the previous comparison results,  \ours (both versions) greatly outperforms all the competing multi-fidelity and single-fidelity methods, confirming the advantage of \ours in predicting complex physical simulation results.  

\subsection{Interpolation and Extrapolation in Fidelities}

Since our method predicts the output as a function of the (continuous) fidelity,  it can predict solution fields at arbitrary fidelities that are different from the training fidelities, namely, interpolation and extrapolation. Note that, the current finite fidelity approaches lack a mechanism to make such predictions. To examine the performance of our model in interpolating and extrapolating the fidelity of  solution prediction, we tested on Poisson's and Heat equation. We generated the four-fidelity training data, including $256$, $128$, $64$, and $32$ examples for the first, second, third and fourth fidelity. The corresponding mesh size is $8 \times 8$, $16 \times 16$, $32 \times 32$ and $64 \times 64$, respectively. The lowest fidelity is $m=0$, and highest $m=1$. We then trained our model, and predicted the solution at $m>1$, which corresponds to denser meshes. For example, $m=1.29, 1.57, 2.14$ correspond to the mesh size $80 \times 80$, $96 \times 96$ and $128 \times 128$.  We viewed the ideal solution as solved using the $128 \times 128$ mesh, with which we generated 256 test examples. We then varied $m \in [0, 2.14]$, and examined the prediction error of \ours at various fidelities. The results are shown in Fig. XX. As we can see, within the range of the training fidelity ($m \le 1$), the prediction error of  \ours-GPODE is consistently smaller than that of  \ours-ODE$^2$, especially at very low fidelities. The best prediction error of \ours-GPODE is achieved at $m=1$, \ie the highest training fidelity. When $m>1$, the performance of \ours-GPODE drops evidently. By contrast, while when $m<1$, the prediction error of \ours-ODE$^2$ is slightly worse than \ours-GPODE, when $m>1$, the performance of \ours-ODE$^2$ keeps improving. At the end $m=2.14$, the prediction error is even better than the best error of \ours-GPODE. It shows that \ours-GPODE is better in interpolation but \ours-ODE$^2$ is promising in extrapolation. This might be attributed to the GP prior used \ours-GPODE, which is known to interpolate well yet not good at extrapolation. The improved extrapolation performance of \ours-ODE$^2$ can be particularly useful in practice. It allows us to train the surrogate model only using relatively low-fidelity examples, but we can still expect to extrapolate predictions to higher fidelities. Therefore, we can avoid generating those higher-fidelity examples for training and hence greatly reduce the cost. 



==> method.tex <==

\section{Background}

%problem definitions 
\textbf{Problem setting.}  We assume that we can query training examples with $M$ fidelities, which correspond to $M$ mappings, $\{\f_m(\x) \in \mathds{R}^{d_m}\}_{1 \le m \le M}$ where $\x \in \Xcal$ is an $r$-dimensional input, $r$ is small, $d_m$ is the output dimension, often very large, and $\{d_m\}$ are not necessarily identical.  In general, we assume $d_1 \le \ldots \le d_M$.  For instance, in structure design, the input can be  the design parameters. The high fidelity examples correspond to high-resolution structures while the low fidelity ones low-resolution structures.  We denote  by $\lambda_m$ the cost to query with fidelity $m$.  To perform active learning, we begin with a small set of training examples with mixed fidelities. Each step, we select both the fidelity and input location to query new training examples, so as to best balance the learning improvement and computational cost, namely, maximizing the benefit-cost ratio. 
%Assume we can query training examples at different fidelites. Th 
%Note that this is different from popular active learning settings that assume a pool of unlabeled input examples, \eg images. Each time, we only need to rank the inputs and select the top examples to query. 
%Traditional active learning assumes a pool of unlabeled input examples, \eg images. Each time,  these examples will be ranked according to some acquisition (or utility) function computed based on the current model.  We expect the top examples will mostly improve the learning performance. We query the labels of these examples, and add them into the training set to update our model.  

\textbf{Dropout active learning.} A very successful application of active learning with deep neural networks is image classification~\citep{gal2017deep,kirsch2019batchbald}. Typically, a pool of unlabeled input examples, \ie images,  is pre-collected. Each time, we rank the input examples according to an acquisition function computed based on the current model. We then query the labels of the top examples, and add them into the training set. There are two popular acquisition functions. The first one is the predictive entropy of the label, 
\begin{align}
	\mathbb{H}[y|\x, \Dcal] = -\sum_{c} p(y=c|\x, \Dcal) \log p(y=c|\x, \Dcal), \label{eq:image-ac-1}
\end{align}
where $\x$ is the input, and $\Dcal$ are the training data. The other one is BALD (Bayesian active learning by disagreement)~\citep{houlsby2011bayesian} --- the mutual information between the label and model parameters, 
\begin{align}
	\mathbb{I}[y, \btheta|\x, \Dcal]  = \mathbb{H}[y|\x, \Dcal]- \EE_{p(\btheta|\Dcal)}\left[\mathbb{H}(\y|\x, \btheta, \Dcal)\right], \label{eq:image-ac-2}
\end{align}
where $\btheta$ are the NN weights. The computation of these acquisition functions require us to first estimate the posterior of the NN output and weights. A popular approach is to use Monte-Carlo (MC) Dropout~\citep{gal2016dropout}, which can be viewed as a variational inference method of Bayesian NNs. MC Dropout uses a probability $p_i$ to randomly drop the neurons in each layer $i$ (equivalent to zeroing out the corresponding weights) in the forward pass and performs backward pass over the remaining neurons. After training, the weights and output obtained from one such forward pass can be viewed as a sample of the approximate posterior. We can run Dropout multiple times to collect a set of posterior samples and calculate the acquisition functions by Monte-Carlo approximation. 

\vspace{-0.05in}
\section{Deep Multi-Fidelity Modeling for High-Dimensional Outputs}
\vspace{-0.05in}
%summarize the problem, and then proceed.
%Despite the success of Dropout active learning, it can be too expensive for high-dimensional outputs. 
%When the output is a high-dimensional (continuous) vector, it is natural to assume a multivariate Gaussian posterior. The entropy  in XX and XX requires the log determinant of the covariance matrix. However, 
Despite its success, dropout active learning might be inappropriate for high-dimensional (continuous) outputs. When the output is a continuous vector, it is natural to use a multivariate Gaussian posterior, $p(\y|\x, \Dcal) \approx \N(\y|\bmu(\x), \bSigma(\x))$, and the entropy $\mathbb{H}(\y|\x, \Dcal)$ in the acquisition functions  (see \eqref{eq:image-ac-1} and \eqref{eq:image-ac-2}) require us to compute the log determinant of the covariance matrix, $\log|\bSigma(\x)|$. While we can use dropout samples to construct an empirical  estimate $\widehat{\bSigma}(\x)$, due to the large output dimension $n$, the computation of this $n\times n$ matrix and its log determinant is very expensive  or even infeasible. 
One might seek to only estimate the variance of each individual output. However, this will ignore the strong, complex output correlations, which is critical to effectively evaluate the uncertainty and calculate the acquisition function. Furthermore, in our active learning task, we want to optimize the acquisition function to find the best input (rather than rank the inputs in a pre-collected pool). The empirical covariance estimation from random samples can lead to numerical instability in optimization and inconsistent results from different runs. 

To overcome these problems for multi-fidelity active learning, we propose a highly expressive deep multi-fidelity model, for which we develop a structural variational inference method to capture the posterior dependency of the outputs. We propose a novel acquisition function to allow multi-fidelity queries, and develop an efficient, tractable, and reliable approach to calculate the acquisition function. 


Specifically, we use deep neural networks to build a multi-fidelity high-dimensional output model (see Fig. \ref{fig:graphical}) that can flexibly, efficiently capture various complex relationships between the outputs and between the fidelities, taking advantage of these relationships to enhance the predictive performance at the highest fidelity (where we make final predictions).  For each fidelity $m$, we introduce a neural network (NN) that first generates a  $k_m$ dimensional  latent output, and then projects it to the $d_m$ dimensional observed vector, where $k_m \ll d_m$. The NN is parameterized by $\{\W_m, \btheta_m, \A_m\}$ where $\W_m$ is a $k_m \times l_m$ weight matrix in the latent output layer, $\A_m$ is a $d_m \times k_m$ projection matrix, and $\btheta_m$ the weights in all the other layers. Denote by $\x_m$ the NN input, by $\f_m(\x)$ the latent NN output, and by $\y_m(\x)$ the observation. The model is defined by
\begin{align}
	\x_m &= 			[\x; \f_{m-1}(\x)],  \notag \\
	%\x_m &= \begin{matrix*}[l] \x, \;\;(m=1)\\ [\x; \f_{m-1}(\x)],\;\;m>1 \end{matrix*} \notag \\
	%\x_m & = \begin{cases}
	%		\x & m=1,\\
	%		[\x; \f_{m-1}(\x)] & m>1,
	%	\end{cases} \notag \\
	\f_m(\x) &= \W_m\bphi_{\btheta_m}(\x_m),\notag \\
	\y_m(\x) &= \A_m \f_m(\x) + \bepsilon_m, \label{eq:our-model}
\end{align}
where $\bphi_{\btheta_m}$ is the $l_m$ dimensional input to the latent output layer (therefore parameterized by $\btheta_m$), and $\bepsilon_m \sim \N(\bepsilon_m|\0, \sigma^2_m\I)$ is an isotropic Gaussian noise. We set $k_0 = 0$ and so $\f_0(\x)$ is empty; when $m=1$, we have $\x_m = \x$. Note that $\bphi_{\btheta_m}$ can be viewed as a set of nonlinear basis functions. Through their combinations via $\W_m$ and $\A_m$, we can flexibly capture  the complex, strong relationships between the elements of $\y_m$ to improve the prediction. Furthermore,  the input $\x_{m}$ is constructed by appending to the original input $\x$  the latent output $\f_{m-1}$, which can be viewed as a compact  (or low-rank) summary of all the information up to fidelity $m-1$.  After a series of linear and nonlinear transformations, we obtain the latent output $\f_m$ --- the summary up to fidelity $m$ --- and then generate the high dimensional observation $\y_m$. In this way, we efficiently integrate the information from lower fidelities and capture the complex relationship between the current and previous fidelities by learning a nonlinear mapping, $\f_m(\x) = h(\x, \f_{m-1}(\x))$, where $h(\cdot)$ is fulfilled by an NN. %When $m=1$, we set $\x_m = \x$. %The graphical illustration of our model is in Fig. \ref{fig:graphical}.
\begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{./graphic}
	\caption{\small Graphical representation of the deep multi-fidelity model. The low dimensional latent output in each fidelity $\f_m(\x)$ ($1\le m \le M$) is generated by a (deep) neural network.} \label{fig:graphical}
	\vspace{-0.15in}
\end{figure}

%Through a series of linear and nonlinear transformations inside
%the NN, we obtain the output fm(x). In this way, we digest the information from the lower fidelities,
%and capture the complex relationships between the current and previous fidelities by learning a
%nonlinear mapping fm (x) = h(x, fm−1 (x)), where h(·) is fulfilled by the NN. When m = 1, we set
%xm = x. A graphical representation of our model is given in Fig. 1 of the supplementary material.

We place a standard Gaussian prior over the elements in each $\W_m$. Similar to~\citep{snoek2015scalable}, we consider all the remaining parameters as hyper-parameters to ease the posterior inference and uncertainty reasoning. Given the training dataset $\Dcal = \{\{(\x_{nm}, \y_{nm})|m\}_{n=1}^{N_m}\}_m$, the joint probability  of our model is given by
\begin{align}
	&p(\Wcal, \Ycal|\Xcal, \Theta, \s) = \prod\nolimits_{m=1}^M \N\left(\vec(\W_m)|\0, \I\right)\notag \\
	&\cdot \prod\nolimits_{n=1}^{N_m} \N\big(\y_{nm}|\A_m \f_m(\x_{nm}), \sigma_m^2\I\big), \label{eq:joint-prob}
\end{align}
where $\Wcal = \{\W_m\}_{1\le m\le M}$,  $\Theta=\{\btheta_m, \A_m\}_{1\le m \le M}$, $\s = [\sigma^2_1, \ldots, \sigma^2_M]^\top$, and $\{\Xcal$, $\Ycal\}$ are the inputs and outputs in $\Dcal$. 

To estimate the posterior of our model (which is used to calculate the acquisition function and query new examples), we develop a stochastic structural variational learning algorithm. Specifically, for each $\W_m$,  we introduce a multivariate Gaussian posterior, $q(\W_m) = \N\left(\vec(\W_m)|\bmu_m, \bSigma_m\right)$.  To ensure the positive definiteness, we parameterize  $\bSigma_m$ by its Cholesky decomposition, $\bSigma_m = \L_m \L_m^\top$, where $\L_m$ is a lower triangular matrix. We then assume the posterior $q(\Wcal) =\prod_{m=1}^M q(\W_m)$, and construct a variational model evidence lower bound (ELBO)~\citep{wainwright2008graphical}, %$\Lcal\big(q(\Wcal), \Theta, \s\big) = \EE_{q}[ \log(p(\Wcal, \Ycal|\Xcal, \Theta, \s)/q(\Wcal))]$. 
\begin{align}
	&\Lcal\big(q(\Wcal), \Theta, \s\big) = \EE_{q}\left[ \log\frac{p(\Wcal, \Ycal|\Xcal, \Theta, \s)}{q(\Wcal)}\right] \notag \\
	&=-\text{KL}\big(q(\Wcal)\|p(\Wcal)\big) \notag \\
	&+ \sum_{m=1}^M\sum_{n=1}^{N_m} \EE_q\left[\log \N(\y_{nm}|\A_m \f_m(\x_{nm}),\sigma_m^2\I)\right], \label{eq:elbo}
\end{align}
where $\text{KL}(\cdot \| \cdot)$ is Kullback Leibler divergence and $p(\Wcal)$ the prior of $\Wcal$. We maximize $\Lcal$ to jointly estimate $q(\Wcal)$ and the hyper-parameters. While $\Lcal$ is intractable, it is straightforward to use the reparameterization trick~\citep{kingma2013auto} to generate parameterized samples for each $\vec(\W_m)$: $\bmu_m + \L_m \bxi_m$ where $\bxi_m \sim \N(\0, \I)$, substitute them into \eqref{eq:elbo} to obtain a stochastic estimate of $\Lcal$,  and perform efficient stochastic optimization. %We left the details in the supplementary material. 

%multi-fidelit queries
\vspace{-0.1in}
\section{Multi-Fidelity Active Learning}
\vspace{-0.1in}
\subsection{Mutual Information based Acquisition Function}
\vspace{-0.1in}
We now consider how to perform active learning with multi-fidelity queries. We assume that at each fidelity $m$, the most valuable training example is the one that can best improve our final prediction, namely, the prediction at the highest fidelity $M$. 
To this end, we propose our acquisition function based on the mutual information between the outputs at fidelity $m$ and $M$,
\begin{align}
	&a(\x, m)  = \frac{1}{\lambda_m} \mathbb{I}\left(\y_m(\x), \y_M(\x)|\Dcal\right) \label{eq:ac} \\
	&= \frac{1}{\lambda_m} \big(\mathbb{H}(\y_m|\Dcal) +\mathbb{H}(\y_M|\Dcal) - \mathbb{H}(\y_m, \y_M|\Dcal) \big), \notag
\end{align}
%\begin{align}
%	a(\x, m)  &= \frac{1}{\lambda_m} \mathbb{I}\left(\y_m(\x), \y_M(\x)|\Dcal\right), \notag \\
%	&= \frac{1}{\lambda_m} \left(\mathbb{H}(\y_m(\x)|\Dcal) +\mathbb{H}(\y_M(\x)|\Dcal) - \mathbb{H}(\y_m(\x), \y_M(\x)|\Dcal) \right) \label{eq:ac}
%\end{align}
where $\lambda_m>0$ is the cost of querying a training example with fidelity $m$. When $m=M$, we have $a(\x, M) = \frac{1}{\lambda_M} \mathbb{H}\left(\y_M(\x)|\Dcal\right)$ ---  the output entropy.  Therefore, our acquisition function is an extension of the popular predictive entropy principle in conventional active learning.  At each step, we maximize our acquisition function to identify a pair of fidelity and input location that give the biggest benefit-cost ratio.  %Note that we can also adjust the BALD principle [??] in the multi-fidelity setting,  $a_{\text{BALD}} = \frac{1}{\lambda_m}$ However, given all the parameters, the uncertainty of the output only comes form the Gaussian noise, ....

%talk about BALD

%challengen, our method
\vspace{-0.1in}
\subsection{Efficient Acquisition Function Calculation}\label{sect:ac-compute}
\vspace{-0.1in}
To maximize the acquisition function \eqref{eq:ac}, a critical challenge is to compute the posterior of the outputs $\{\y_m\}$ in every fidelity, based on our model estimation results, $p(\Wcal|\Dcal) \approx q(\Wcal)$.  Due to high dimensionality of each $\y_m$ and the nonlinear coupling of the latent outputs across the fidelities (see \eqref{eq:our-model}), the computation is challenging and analytically intractable.  To address this issue, we first consider approximating the posterior of the low dimensional latent output $\f_m$, which can be viewed a function of the random NN weights $\bOmega_m = \{\W_1, \ldots, \W_m\}$ (given the input $\x$). We use multivariate Delta's method~\citep{oehlert1992note,bickel2015mathematical} to compute the moments of $\f_m$. Specifically, we approximate $\f_m$ with a first-order Taylor expansion, 
\begin{align}
	\f_m(\bOmega_m) \approx \f_m(\EE[\bOmega_m]) + \J_m\left(\boldeta_m  - \EE[\boldeta_m]\right), \label{eq:1order}
\end{align}
where the expectation is under $q(\cdot)$,  $\boldeta_m = \vec(\bOmega_m)$, $\J_m = \frac{\partial \f_m}{\partial \boldeta_m}|_{\boldeta_m = \EE[\boldeta_m]}$ is the Jacobian matrix at the mean.  The rationale is as follows. First, $\f_m$ is linear to $\W_m$, and the second-order derivative is simply $\0$.  Second, as the NN output, $\f_m$ is highly nonlinear to the random weights in previous layers, \ie $\W_j$ ($j<m$). Hence, we can assume the change rate of $\f_m$ (\eg gradient or Jacobian) has much greater scales than the posterior covariance of $\W_j$ in the second-order term of the Taylor expansion. Note that $q(\W_j)$ is much more informative and hence much more concentrated than the prior $ \N(\vec(\W_j)|\0, \I)$. The scale of the posterior covariance should be much less than $1$. Integrating both cases, the first-order term can dominate the Taylor expansion and hence we ignore the higher order terms. 
Based on \eqref{eq:1order}, we can easily calculate the first and second moments of $\f_m$, 
\begin{align}
	\balpha_m &= \EE[\f_m] \approx \f_m\left(\EE[\bOmega_m]\right), \notag \\
	\V_m &= \text{cov}[\f_m] \approx \J_m \text{cov}(\boldeta_m) \J_m^\top, 
\end{align}
where  $\text{cov}(\boldeta_m) = \diag\left(\left\{\text{cov}\big(\vec(\W_j)\big)\right\}_{1\le j\le m}\right)$. 
Then we use moment matching to estimate a joint Gaussian posterior, $q(\f_m)  = \N(\f_m|\balpha_m, \V_m)$. Next, according to our model definition \eqref{eq:our-model}, we can obtain the posterior of the ouptut $\y_m$, 
\begin{align}
	q(\y_m) = \N(\y_m|\A_m \balpha_m, \A_m \V_m \A_m^\top + \sigma_m^2\I).
\end{align}
The output entropy is  $\mathbb{H}(\y_m|\Dcal) = \frac{1}{2}\log|\A_m \V_m \A_m^\top + \sigma_m^2\I| + d_m \log\sqrt{2\pi e}$.  However, directly computing the log determinant of a $d_m \times d_m$ matrix is very expensive. We further use the Weinstein-Aronszajn identity~\citep{kato2013perturbation} to derive 
\begin{align}
	&\mathbb{H}(\y_m|\Dcal) =  \frac{1}{2}\log|\sigma_m^{-2}\A_m \V_m \A_m^\top + \I|  + d_m \log \sqrt{2\pi e\sigma_m^2} \notag \\
	&=\frac{1}{2}\log|\sigma_m^{-2}\A_m^\top\A_m\V_m + \I| + d_m \log \sqrt{2\pi e\sigma_m^2}. \label{eq:en_ym}
\end{align}
Now, the log determinant is calculated on a much smaller, $k_m \times k_m$ matrix, which is very cheap and efficient. 

Using a similar approach, we can calculate the joint posterior of $\barf_m = [\f_m; \f_M]$ and then $\bary_m=[\y_m; \y_M]$.  First, we view $\barf_m$ as a function of all the random weights, $\Wcal = \{\W_1, \ldots, \W_M\}$. We use the multivariate Delta's method and moment matching to estimate a joint Gaussian posterior, 
$q(\barf_m) = \N(\barf_m|\baralpha_m, \barV_m)$ where $\baralpha_m = \barf_m\left(\EE[\Wcal]\right)$,  $\barV_m = \barJ_m \text{cov}(\boldeta)\barJ_m^\top$, $\boldeta = \vec(\Wcal)$, $\barJ_m = \frac{\partial \barf_m}{\partial \boldeta}|_{\boldeta = \EE[\boldeta]}$, and $\text{cov}(\boldeta) = \diag\left(\left\{\text{cov}\big(\vec(\W_j)\big)\right\}_{1\le j\le M}\right)$. According to our model, we can represent
\[
\bary_m = \barA_m \barf_m + \bareps_m,
\]
where $\barA_m = \diag(\A_m, \A_M)$ and $\bareps_m = [\bepsilon_m; \bepsilon_M]$. Therefore, the joint posterior of $\bary_m$ is 
\begin{align}
	q(\bary_m) = \N(\bary_m|\barA_m \baralpha_m, \barA_m \barV_m \barA_m^\top + \S_m),
\end{align}
where $\S_m = \diag(\sigma^2_m\I_{d_m}, \sigma^2_M \I_{d_M})$,  $\I_{d_m}$ and $\I_{d_M}$ are identity matrices of $d_m \times d_m$ and $d_M \times d_M$, respectively.  Again, we use  Weinstein-Aronszajn identity to simplify the entropy computation of $\bary_m$ (\ie $\y_m$ and $\y_M$), 
\begin{align}
	&\mathbb{H}(\y_m, \y_M|\Dcal)  =\frac{1}{2}\log|\S_m^{-1}\barA_m \barV_m \barA_m^\top + \I|  + \xi_m \notag \\
	&=\frac{1}{2}\log|\barA_m^\top \S_m^{-1} \barA_m \barV_m + \I| + \xi_m, \label{eq:en_ymM}
\end{align}
where $\xi_m = d_m \log \sqrt{2\pi e\sigma_m^2} + d_M \log \sqrt{2\pi e\sigma_M^2}$ and the log determinant is computed from a $(k_m + k_M) \times (k_m + k_M)$ matrix, which is cheap and efficient. Note that we can use matrix blocks to compute $\barA_m^\top \S_m^{-1} \barA_m = \diag\left(\sigma_m^{-2}\A_m^\top \A_m, \sigma_M^{-2}\A_M^\top \A_M\right)$.

Now, based on \eqref{eq:en_ym} and \eqref{eq:en_ymM}, we can calculate our acquisition function \eqref{eq:ac} in an analytic and deterministic way. For each fidelity $m$, we maximize $a(\x, m)$ w.r.t to $\x$ to find the optimal input. We can use automatic differential libraries to calculate the gradient and feed it to any optimization algorithm, \eg L-BFGS.   We then use the optimal input at the fidelity that has the largest acquisition function value to query  the next training example. Our deep multi-fidelity active learning is summarized in Algorithm \ref{alg:dmf-al}. 
%problem of dropout ... 
\setlength{\textfloatsep}{0.05cm}
\begin{algorithm}                      % enter the algorithm environment
	\small
	\caption{\ours($\Dcal$, $T$, $\{\lambda_m\}_{m=1}^M$ )}          
	\label{alg:dmf-al}                           
	\begin{algorithmic}[1]                    % enter the algorithmic environment
		\STATE Train the deep multi-fidelity model \eqref{eq:joint-prob} on the initial dataset $\Dcal$ with stochastic structural variational learning.  
		\FOR {$t=1,\ldots, T$}
		\STATE Based on \eqref{eq:en_ym} and \eqref{eq:en_ymM}, calculate and optimize the acquisition function \eqref{eq:ac} to find 
		\begin{align}
			(\x_{t}, m_{t}) = \argmax_{\x \in \Xcal, 1\le m \le M} a(\x, m).\notag % =  \frac{1}{\lambda_m} \mathbb{I}\left(\y_m(\x), \y_M(\x)|\Dcal\right).\notag
		\end{align}
		\STATE Query the output $\y_{t}$ with fidelity $m_t$.
		\STATE $\Dcal \leftarrow \Dcal \cup \{(\x_{t}, \y_{t})|m_t\}$.
		\STATE Re-train the deep multi-fidelity model on $\Dcal$.
		\ENDFOR
		%\vspace{-0.05in}
		%\RETURN the current posterior $q_{cur}(\cdot)$.
	\end{algorithmic}
\end{algorithm}
\setlength{\floatsep}{0.1cm}
\vspace{-0.05in}
\subsection{Algorithm Complexity}
\vspace{-0.05in}
The time complexity of training our deep multi-fidelity model is $\Ocal(N(\sum_{m=1}^M (k_ml_m)^2 + F))$ where $N$ and $F$ are the total number of training examples and NN parameters, respectively. The space complexity is $\Ocal(F + \sum_{m=1}^M (k_ml_m)^2)$, which is to store the NN parameters, and posterior mean and covariance of each random weight matrix $\W_m$. The time complexity of calculating the acquisition function is $\Ocal(\sum_{m=1}^M d_mk_m^2 + k_m^3)$. Since $k_m \ll d_m$, the complexity is linear to the output dimensions. Due to the usage of the learned variational posterior $q(\Wcal)$, the space complexity of computing the acquisition function is the same as that of training the multi-fidelity model.

